Understanding Time Variations of DNN Inference in Autonomous Driving

Deep neural networks (DNNs) are widely used in autonomous driving due to their high accuracy for perception, decision, and control. In safety-critical systems like autonomous driving, executing tasks like sensing and perception in real-time is vital to the vehicle's safety, which requires the application's execution time to be predictable. However, non-negligible time variations are observed in DNN inference. Current DNN inference studies either ignore the time variation issue or rely on the scheduler to handle it. None of the current work explains the root causes of DNN inference time variations. Understanding the time variations of the DNN inference becomes a fundamental challenge in real-time scheduling for autonomous driving. In this work, we analyze the time variation in DNN inference in fine granularity from six perspectives: data, I/O, model, runtime, hardware, and end-to-end perception system. Six insights are derived in understanding the time variations for DNN inference.

==> 4_time_modeling.tex <==
\label{time-model}
The time variations in DNN inference brings an essential challenge for the time modeling of DNN inference. In this section,  we first present a generalized pipeline of a representative object and lane detection models. Next, based on the analysis and insights of DNN inference time variations in Section~\ref{profiling}, we propose a DNN inference time prediction model which leverages the intermediate results to predict the end-to-end latency of DNN inference. Finally, we show the performance of the DNN inference time models on the KITTI dataset.

\subsection{Detection Pipeline}

A generalized object and lane detection pipeline is shown in Figure~\ref{fig:detection-pipeline}. Generally, the detection pipeline starts with the sensor data access and pre-processing of the raw data. For image-based object and lane detection, the pre-processing contains \textit{resize} and \textit{transform} operations pre-defined by the model training process. The output of pre-processed sensor data will be fed into the inference engine for feature extraction and post-processing for final detection results. In this 
section, we focus on two-stage based object detection models, which cover R-CNN, Fast R-CNN, Faster R-CNN, Mask R-CNN, etc.~\cite{girshick2014rich,girshick2015fast,ren2015faster,he2017mask} Besides, the lane detection pipeline is generalized from state-of-the-art works, including LaneNet, PINet, etc.~\cite{neven2018towards,ko2020key}

\textbf{Object detection.} 
For two-stage based object detection algorithms, the backbone like ResNet~\cite{he2016deep} or VGG~\cite{simonyan2014very} is used to extracted features from the pre-processed image data and create feature maps. Then the first stage goes through the Region Proposal Network (RPN), which creates region proposals based on a softmax layer to classify anchors as objects or backgrounds and uses bounding box regression to fix the proposals. The second stage starts with Region of Interest (RoI) pooling which collects features maps and region proposals to extract proposal feature maps. Then they are submitted to the classifier, which has fully connected layers to get the proposal's object class and fixed bounding box. The inference covers all the modules from the backbone to the classifier, and it is usually executed on GPU. Post-processing operations include bounding box transformation and drawing bounding boxes on the original image.

\textbf{Lane detection.} 
The network in lane detection models starts with feature extraction, which contains an encoder-decoder structure like the hourglass block to create feature maps. Then two segmentation branches will be leveraged to get the pixel-wise lane proposals. Binary segmentation outputs the pixels belonging to lanes, while instance segmentation branch outputs which lane each pixel belongs. By combining the results from these two branches, raw lane points are generated. Post-processing contains the clustering of raw lane points and lane fitting results.

\begin{figure}[!htp]
	\centering
	\includegraphics[width=.8\columnwidth]{figures/PDNN/PDNN-flow.pdf}
	\caption{Generalized object and lane detection pipelines.}
	\label{fig:detection-pipeline}
\end{figure}

% \begin{figure}[!htp]
% 	\centering
% 	\includegraphics[width=\columnwidth]{figures/PDNN/proposal-post-processing.pdf}
% 	\caption{The time sequence and correlation coefficients of proposals and DNN inference post-processing time.}
% 	\label{fig:proposal-post}
% \end{figure}

\subsection{Proposal-based Detection Time Modeling}

Based on the findings in Section~\ref{profiling}, we know that the DNN inference time variations are mainly caused by post-processing, while time variations of the other processes are negligible. Besides, since the operations in post-processing are closely related to the intermediate results in inference, finding the mathematical relationship between post-processing and inference becomes the key to predict model end-to-end DNN inference time. The proposed DNN end-to-end time modeling contains two parts: static time modeling, dynamic time modeling.

\textbf{Static time modeling.}
The static time modeling is based on collected logs to find the distribution and relationship for each component within the DNN inference. To begin with, we collected logs of DNN models with fine-grained breakdowns, and some intermediate inference results include the proposal. As we have seen in Figure~\ref{fig:proposal-post}, the post-processing time correlates with the number of proposals. This finding inspires us to leverage the number of proposals from the RPN to predict the post-processing time. Therefore, we use the number of proposals to predict the post-processing time, which turns out to be linear regression. Besides, for remaining time in read, pre-processing, and inference, we leverage a narrow Gaussian distribution with collected logs for prediction since the time variations are limited. Similarly, in lane detection, the raw points generated from two segmentation branches can be seen as lane point proposals, which can be leveraged to predict the follow-up post-processing time, which contains huge time variations. For the clustering process, since it requires calculating all the neighbors of the pixels, we believe there would be a polynomial relationship between proposals and clustering time. By checking the source code and fitting different orders of polynomial regression of the lane proposals with post-processing time, second-order polynomial regression is leveraged for prediction.

\begin{equation}
\label{equ:time-model}
    \left\{
             \begin{array}{lr}
            %  P(T_{r}^{(n)}) = \frac{1}{\sigma \sqrt{2\pi }}e_{}^{-\frac{1}{2}(\frac{x-\mu }{\sigma })^{2}} \\

T_{r}^{(0)} = \frac{\sum t_{r}^{0}}{m}, 

T_{r}^{(n)} = \frac{\sum t_{r}^{n}}{m} \\

T_{1}^{(n)} = \alpha_{1} p^{(n)} + \alpha _{0} \\

T_{2}^{(n)} = \beta_{2} (l^{(n)})^{2} +\beta_{1} l^{(n)}+ \beta _{0} \\

T_{OD}^{(n)} = \lambda (T_{1}^{(n)} + T_{r}^{(0)}) \\

T_{LD}^{(n)} = \lambda (T_{2}^{(n)} + T_{r}^{'(0)}) \\

\lambda = \frac{T_{r}^{0}}{T_{r}^{n}}
             \end{array}
\right.
\end{equation}

\textbf{Dynamic time modeling.}
In addition to static time modeling, we also introduce a calibration factor $\lambda$ which reflects the dynamic time modeling caused by the devices' runtime conditions (temperatures, etc.)~\cite{wan2020alert}. The calibration factor reflects the relative runtime performance compared with the time when logs are collected. With the adjustment of prediction time from the static time modeling, the final prediction for end-to-end DNN inference time is generated. 

% \textcolor{red}{Say something before jumping to Eqn. (4)}

The Equation~(\ref{equ:time-model}) contains the end-to-end inference time model for object detection and lane detection. $T_{r}^{(0)}$ represents the remaining inference time (read, preprocessing, and inference) for collected logs, while $T_{r}^{(n)}$ represents the current remaining inference time. By dividing these two values, we can get the calibration factor $\lambda$. $T_{1}^{(n)}$ represents the current post-processing time for object detection, where $p^{(n)}$ is the number of proposals from current inference task. $T_{1}^{(n)}$ represents the current post-processing time for lane detection, where $l^{(n)}$ is the number of lane pixels in the current inference task. Parameters $\alpha$ and $\beta$ represent the regression weights, and they are learned from collected logs. Finally, the end-to-end latency is modeled as the summation of the current post-processing time and remaining time multiplying the calibration factor $\lambda$.

\subsection{Evaluation}

To evaluate the performance of the proposed DNN end-to-end inference time model, we collect logs when running models on the image dataset and train the weights for Faster R-CNN, LaneNet, and PINet. Figure~\ref{fig:time-model-results} shows the results for ground truth and predicted end-to-end latency. We can observe that the prediction line aligns very well with the ground truth line over all the 600 images. 

We collect the prediction results and calculate the absolute error and prediction accuracy for each image. The results are shown in Table~\ref{tab:model-results}. We can observe that the prediction for Faster R-CNN performs the best, which has 98.99 percent accuracy and less than 3.5ms average error. Both LaneNet and PINet have accuracy higher than 90 percent, while the average errors are less than 24ms. However, the prediction error is still acceptable compared with the DNN time variation range which is even larger than 263ms for LaneNet and PINet. 

\begin{figure}[!htp]
	\centering
	\includegraphics[width=.6\columnwidth]{figures/PDNN/time-model-results.pdf}
	\caption{The ground truth (real) results and predicted end-to-end latency for Faster R-CNN, LaneNet, and PINet.}
	\label{fig:time-model-results}
\end{figure}

\begin{table}
\centering
\caption{The average real/predicted end-to-end latency, errors, and accuracy for three models.}
\label{tab:model-results}
\resizebox{.6\linewidth}{!}{%
\begin{tabular}{ccccc} 
\toprule
\textbf{Model} & \textbf{Real (ms)} & \textbf{Predicted (ms)} & \textbf{Error (ms)} & \textbf{Accuracy (\%)} \\ 
\hline
\textit{Faster R-CNN} & 321.79 & 321.76 & 3.28 & \textbf{98.99} \\
\textit{LaneNet} & 152.66 & 152.39 & 9.87 & \textbf{94.03} \\
\textit{PINet} & 253.23 & 237.20 & 23.10 & \textbf{91.68} \\
\bottomrule
\end{tabular}
}
\end{table}
